Climate Model Tuning with Online Synchronization-Based Parameter Estimation

In climate science, the tuning of climate models is a computationally intensive problem due to the combination of the high-dimensionality of the system state and long integration times. Supermodelling is a technique which has shown the potential for reducing climate model biases by dynamically coupling multiple models together, and training their coupling on a short timescale. Here, we introduce a new approach called \emph{adaptive supermodeling}, where the internal model parameters of the member of a supermodel are tuned. We perform three experiments. We first directly optimize the internal parameters of a climate model. We then optimize the weights between two members of a supermodel in a classical supermodel approach. For a case designed to challenge the two previous methods, we implement adaptive supermodeling, which achieves a performance similar to a perfect model.

==> climerror_report_exppaper3_2A.tex <==
\begin{tabular}{lrr}
\toprule
 & RMSE mean u & RMSE \sigma u \\
\midrule
Truth & 0.000000 & 0.000000 \\
Observation & 0.000000 & 0.000000 \\
Model 2 & 4.321677 & 4.115128 \\
\bottomrule
\end{tabular}


==> climerror_report_exppaper3_2B.tex <==
\begin{tabular}{lrr}
\toprule
 & RMSE mean u & RMSE \sigma u \\
\midrule
Truth & 0.000000 & 0.000000 \\
Observation & 0.000000 & 0.000000 \\
Model 2 & 4.530237 & 1.641221 \\
\bottomrule
\end{tabular}


==> climerror_report_exppaper3_3A.tex <==
\begin{tabular}{lrr}
\toprule
 & RMSE mean u & RMSE \sigma u \\
\midrule
Truth & 0.000000 & 0.000000 \\
Observation & 0.000000 & 0.000000 \\
Model 2 & 4.753810 & 1.760467 \\
\bottomrule
\end{tabular}


==> climerror_report_exppaper3_3B.tex <==
\begin{tabular}{lrr}
\toprule
 & RMSE mean u & RMSE \sigma u \\
\midrule
Truth & 0.000000 & 0.000000 \\
Observation & 0.000000 & 0.000000 \\
Model 2 & 1.514487 & 0.945943 \\
\bottomrule
\end{tabular}


==> climerror_report_exppaper3_3D.tex <==
\begin{tabular}{lrr}
\toprule
 & RMSE mean u & RMSE \sigma u \\
\midrule
Truth & 0.000000 & 0.000000 \\
Observation & 0.000000 & 0.000000 \\
Model 2 & 4.525009 & 2.092220 \\
Model 3 & 4.525009 & 2.092220 \\
SUMO & 4.525009 & 2.092220 \\
\bottomrule
\end{tabular}


==> climerror_report_exppaper3_5A.tex <==
\begin{tabular}{lrr}
\toprule
 & RMSE mean u & RMSE \sigma u \\
\midrule
Truth & 0.000000 & 0.000000 \\
Observation & 0.000000 & 0.000000 \\
Model 2 & 0.123681 & 0.237064 \\
Model 3 & 0.123681 & 0.237064 \\
SUMO & 0.123681 & 0.237064 \\
\bottomrule
\end{tabular}


==> climerror_report_exppaper3_5B.tex <==
\begin{tabular}{lrr}
\toprule
 & RMSE mean u & RMSE \sigma u \\
\midrule
Truth & 0.000000 & 0.000000 \\
Observation & 0.000000 & 0.000000 \\
Model 2 & 0.254482 & 0.264852 \\
Model 3 & 0.254482 & 0.264852 \\
SUMO & 0.254482 & 0.264852 \\
\bottomrule
\end{tabular}


==> climerror_report_exppaper4_3B.tex <==
\begin{tabular}{l}
\toprule
\midrule
\bottomrule
\end{tabular}


==> climerror_report_exppaper4_5B.tex <==
\begin{tabular}{lrrrr}
\toprule
 & RMSE mean u & RMSE error mean u & RMSE \sigma u & RMSE error \sigma u \\
\midrule
Truth & 0.000000 & 0.000000 & 0.000000 & 0.000000 \\
Observation & 8.881764 & 0.015103 & 7.872806 & 0.027957 \\
Model 2 & 8.881764 & 0.015103 & 7.872806 & 0.027957 \\
Model 3 & 8.881764 & 0.015103 & 7.872806 & 0.027957 \\
SUMO & 0.574285 & 0.069794 & 0.255738 & 0.016215 \\
\bottomrule
\end{tabular}


==> params_endvals_exppaper4_3A.tex <==
\begin{tabular}{lr}
\toprule
 & 2 \\
\midrule
dis & 0.000000 \\
addisl & -1.571122 \\
addish & -0.136308 \\
dif & -0.625009 \\
rel & 0.020898 \\
rh0 & -0.031637 \\
\bottomrule
\end{tabular}


==> params_endvals_exppaper4_3B.tex <==
\begin{tabular}{lr}
\toprule
 & 2 \\
\midrule
dis & 4.499970 \\
addisl & 1.173000 \\
addish & 0.681960 \\
dif & 7.000129 \\
rel & 44.352620 \\
rh0 & 8.952551 \\
\bottomrule
\end{tabular}


==> params_endvals_exppaper4_3D.tex <==
\begin{tabular}{lrrr}
\toprule
 & SUMO & 2 & 3 \\
\midrule
weight & 0.120690 & NaN & NaN \\
dis & 4.499970 & 4.499970 & 4.499970 \\
addisl & 0.500000 & 0.500000 & 0.500000 \\
addish & 0.500000 & 0.500000 & 0.500000 \\
dif & 6.336318 & 1.499990 & 7.000129 \\
rel & 19.999867 & 19.999867 & 19.999867 \\
rh0 & 9.000090 & 9.000090 & 9.000090 \\
\bottomrule
\end{tabular}


==> params_endvals_exppaper4_5A.tex <==
\begin{tabular}{lrr}
\toprule
 & 2 & 3 \\
\midrule
dis & 0.000000 & 0.000000 \\
addisl & -0.345370 & 0.000000 \\
addish & -0.179871 & 0.000000 \\
dif & -0.625009 & 0.750000 \\
rel & -1.259528 & -0.555556 \\
rh0 & -0.036089 & 0.000000 \\
\bottomrule
\end{tabular}


==> params_endvals_exppaper4_5B.tex <==
\begin{tabular}{lrrr}
\toprule
 & SUMO & 2 & 3 \\
\midrule
weight & 0.204170 & NaN & NaN \\
dis & 4.499970 & 4.499970 & 4.499970 \\
addisl & 0.567908 & 0.500000 & 0.585330 \\
addish & 0.559592 & 0.500000 & 0.574880 \\
dif & 5.877166 & 1.499990 & 7.000129 \\
rel & 56.818937 & 19.999867 & 66.264861 \\
rh0 & 8.862264 & 9.000090 & 8.826904 \\
\bottomrule
\end{tabular}

